GMKF: Generalized Moment Kalman Filter for Polynomial Systems with Arbitrary Noise

This paper develops a new filtering approach for state estimation in polynomial systems corrupted by arbitrary noise, which commonly arise in robotics. We first consider a batch setup where we perform state estimation using all data collected from the initial to the current time. We formulate the batch state estimation problem as a Polynomial Optimization Problem (POP) and relax the assumption of Gaussian noise by specifying a finite number of moments of the noise. We solve the resulting POP using a moment relaxation and prove that under suitable conditions on the rank of the relaxation, (i) we can extract a provably optimal estimate from the moment relaxation, and (ii) we can obtain a belief representation from the dual (sum-of-squares) relaxation. We then turn our attention to the filtering setup and apply similar insights to develop a GMKF for recursive state estimation in polynomial systems with arbitrary noise. The GMKF formulates the prediction and update steps as POPs and solves them using moment relaxations, carrying over a possibly non-Gaussian belief. In the linear-Gaussian case, GMKF reduces to the standard Kalman Filter. We demonstrate that GMKF performs well under highly non-Gaussian noise and outperforms common alternatives, including the Extended and Unscented Kalman Filter, and their variants on matrix Lie group.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> logic.tex <==
\section{Logic}
\harry{LC comments to be addressed...}
\begin{enumerate}
    \item Problem statement: filtering of polynomial dynamical systems
    \item Polynomial KF: procedural presentation of propagation and update, and give some intuition about why they make sense and the fact that there is no longer a closed-form solution but we need to solve optimization problems.
    \item For r=1 and Gaussian noise this becomes KF
    \item Show why it makes sense, in particular: (i) BPUE vs BLUE, (ii) why covariance can be "approximately" extracted from the dual, (iii) show marginalization for the propagation step.
    
\end{enumerate}
Furthermore, we provide both quantitative and qualitative results that demonstrate the effectiveness of our proposed filtering technique on highly nonlinear dynamical systems with highly non-Gaussian noises. 
\harry{Look for missing Experiments}:
\begin{enumerate}
    \item prediction: show that after prediction GKF produces a banana-shaped distribution, while EKF produces a less accurate distribution (see this for inspiration: https://www.roboticsproceedings.org/rss08/p34.pdf)
    \item update step: BPUE ablation: linear case, binary/non-gaussian noise, evaluation of covariances (and show they empirically make sense)
    \item do just a localization experiment comparing with EKF and using a very nonlinear measurement model, e.g., range only or range/bearing + motion in SE(2). some serious ablation on noise magnitude. Maybe use Victoria Park but with fixed landmarks: \url{https://www.mrpt.org/Dataset_The_Victoria_Park} (or a 2D localization dataset? google: "landmark-based 2D localization"). 
\end{enumerate}

\begin{equation}
     T_k^{-1}X_k^{-1}X_{k+1} = w_k
\end{equation}
% \begin{abstract}

% \end{abstract} 

% \IEEEpeerreviewmaketitle
% \begin{enumerate}[1.]
%     \item Define the BPUE as a optimization on rank-one ``moment'' matrix, thus we have the notion of tangent space and the covariance in the tangent space.
%     \item Solve the BPUE using SDP relaxation. Show the generalized Kalman gain. Then we have the update of the covariance at the limiting case (at the same tangent space). % \tsl{The vector transport? } 
%     \item Once we have the covariance defined in tangent space, we can marginalize by extracting the sub-principle matrix of the rank-one moment matrix. 
% \end{enumerate}
\tsl{TODO: About the presentation. }
\begin{enumerate}
    \item Define BPUE as BLUE plus QCQP moment matrix constraints.
    \item Solve the BPUE using SDP relaxation. Show the generalized Kalman gain. Then we have the update of the covariance at the limiting case (at the same tangent space). % \tsl{The vector transport? } 
    \item Once we have the covariance defined in tangent space, we can marginalize by extracting the sub-principle matrix of the rank-one moment matrix. 
\end{enumerate}


==> tex/BPUE_old.tex <==
\section{Batch Estimation in Polynomial Systems \\ with Arbitrary Noise}
\label{sec:BPUE}

In this section, we consider a batch setup where we are given measurements from time $0$ to current time $N$ and our goal is to estimate the state ${\M x}_0, \ldots, {\M x}_{N}$.
%show how to incorporate higher-order moments of the noise into the polynomial state-space model and design an optimal filter, dubbed the Generalized Moment Kalman Filter (GMKF), for state estimation using moment relaxation. 
We first show how to account for the higher-order moments of the noise (Section~\ref{sec:extendedPolySys}) and then derive an optimal estimator (Section~\ref{sec:BPUEdetails}). 
For the remainder of the paper, {\color{red} we use $\bar{(\cdot)}$ to denote the true state} and $\hat{(\cdot)}$ for the estimated state. 
% \textcolor{blue}{(Ashkan: Try using a top-down approach instead of a bottom-up one when explaining the GMKF.
% Start with Eq of Figure (1), e.g., to consider higher order moments GMKF minimizes Eq(I): $||\phi(x) - \phi(\hat{x})||^2_{P^{-1}}$ instead of $||x- \hat{x}||^2_{P^{-1}}$. Then start expanding Eq(I) to get to Eq(11) in Problem 1.)}

\subsection{Extended Polynomial Dynamical Systems}
\label{sec:extendedPolySys}
% The classical Kalman filter assumes a linear dynamical system and uses moment information of the noise up to the second order, i.e. the mean and covariance. 
% In our formulation, we make no assumption on the linearity and the Gaussian noise. 
% Instead, we only assume that we know arbitrary moments of the noise. 
To utilize the higher-order moment of noise, we need an extended version of \eqref{eq:polyDynSys} that includes the higher-order {\color{green}terms} of noise in the state space model.
% \begin{definition}[Extended polynomial dynamical system] 
To achieve this goal, we apply $\M \phi_r(\cdot)$ to both sides of eq.~\eqref{eq:polyDynSys} to generate $r$th-order {\color{green}terms} of the noise:
\textcolor{blue}{( Ashkan: Representation (7) introduces higher order terms NOT higher order moments. $\phi_r$ is a vector of polynomial basis NOT moments)}\tsl{Solved.}
\begin{equation}
\begin{aligned}
    \label{eq:ext-polyDynSys}
    &\left\{
	\begin{array}{l}
	\M \phi_r\left(\M f( \M x_{k+1}, \M x_{k}, \M u_k )\right) = \M \phi_r(\M w_k) \\
	\M \phi_r\left(\M h( \M y_k, \M x_{k} )\right) = \M \phi_r(\M v_k) \\
	\end{array}.
\right. \\
\end{aligned}
\end{equation}
Intuitively,~\eqref{eq:ext-polyDynSys} combines the original process and measurement models into higher-order polynomials by taking powers and products of the entries of $f$ and $h$. Below, we refer to $\M \phi_r(\M w_k)$ and $\M \phi_r(\M v_k)$ as the \emph{extended noise}.

To make the estimation unbiased, we subtract the mean of the extended noises on both sides of \eqref{eq:ext-polyDynSys}, resulting in the following ``moment conditions'' of \eqref{eq:ext-polyDynSys} for both dynamics and measurements\footnote{The astute reader may recognize that this is equivalent to the moment conditions imposed in the Generalized Method of Moments \cite{hansen1982large, hayashi2011econometrics}.}: 
\textcolor{blue}{(Ashkan:How did you derive Eq (8)) from Eq(7)?) According to the definition of $\phi_r$, it is a vector of polynomials basis. Why do you call it moments?}\harry{GMM terminology footnote}
\david{(8) is definition rather than by derivation. The moment condition comes from GMM.}
%
\begin{equation}
\label{gmm_condition}
\begin{aligned}
    \M m_{dyn}(\M x_{k+1}, \M x_{k}, \M u_k) &:= \M \phi_r(\M f(\M x_{k+1}, \M x_{k}, \M u_k)) - \mathbb{E}[\M \phi_r(\M w_k)] \\
    \M m_{obs}(\M y_k, \M x_k) &:= \M \phi_r(\M h(\M y_k, \M x_k)) -  \mathbb{E}[\M \phi_r(\M v_k)]
\end{aligned}
\end{equation}
$\M m_{dyn}$ and $\M m_{obs}$ are zero-mean vectors if $\M x_k$ and $\M x_{k+1}$ are taken at the true values $\bar{\M x}_k$ and $\bar{\M x}_{k+1}$. Then, we define the covariance of the extended noise {\color{green} on the RHS of \eqref{gmm_condition}}:
\begin{equation}
\begin{aligned}
    \M Q_r &:= \operatorname{Cov}\left[\left(\M \phi_r(\vw) - \mathbb{E}\left[\M \phi_r(\vw)\right]\right)\right]  \\
    \M R_r &:= \operatorname{Cov}\left[\left(\M \phi_r(\vv) - \mathbb{E}\left[\M \phi_r(\vv)\right]\right)\right]
    % \M R_r &:= \mathbb{E}\left[\left(\M \phi_r(\vv) - \mathbb{E}\left[\M \phi_r(\vv)\right]\right)\left(\M \phi_r(\vv) - \mathbb{E}\left[\M \phi_r(\vv)\right]\right)^{\transpose}  \right] \\
    % \M Q_r &:= \mathbb{E}\left[\left(\M \phi_r(\vw) - \mathbb{E}\left[\M \phi_r(\vw)\right]\right)\left(\M \phi_r(\vw) - \mathbb{E}\left[\M \phi_r(\vw)\right]\right)^{\transpose}  \right]  
\end{aligned}.
\label{RQdef}
\end{equation}

% It is obvious to see they have zero mean value when taking $\M x_{k}$ at the ground truth value $\bar{x}_k$. 

Consider $N$ inputs $\{\M u_0, \M u_1, \cdots, \M u_{N-1}\}$ and measurements $\{\M y_1, \M y_2, \cdots, \M y_N\}$, we formulate the state estimation problem for state $\{\M x_0, \M x_1, \cdots, \M x_N\}$ with the weighting matrices for each moment condition:
\begin{equation}
    {\color{red} \{ \M Q^{-1}_{r, 0}, \M R^{-1}_{r, 0}, \cdots, \M Q^{-1}_{r, N-1}, \M R^{-1}_{r, N-1}\}. % \M P^{-1}_{r, 0},
    }
\end{equation}
\harry{index shifted by 1}

We then define the batch state estimation problem as the following \eqref{prob:pop} to obtain the state estimation $\hat{\M x}$:
\begin{problem}[Batch State Estimation] % \LC{this makes a lot of sense, but it is confusing since we don't actually solve this problem}
\label{prob:filter_batch}
    \begin{equation}
    \begin{aligned}
        \min_{ \{\M x_{0, \dots N} \} }  \sum_{k=0}^{N-1} & \| \M m_{dyn}(\M x_{k+1}, \M x_{k}, \M u_{k})\|^2_{\M Q^{-1}_{r, k}}
        + \| \M m_{obs}(\M y_k, \M x_{k})\|^2_{\M R^{-1}_{r, k}} \\
        + & \| \M \phi_r(\M x_0) - \M \phi_r(\hat{\M  x}_0)\|^2_{\M P^{-1}_{r, 0}} \\
        \mathrm{s.t.} & \quad \M x_{i} \in \mathcal{K}, ~\forall i \in \{0, 1, \dots, N\}.
    \end{aligned}
\end{equation}
where the term $\| \M \phi_r(\M x_0) - \M \phi_r(\hat{\M  x}_0)\|^2_{\M P^{-1}_{r, 0}}$ is a given prior on the initial state at time $0$.
%To consider the initial state, we also include an SOS polynomial for $\M x_0$ in the cost function with the weighting matrix $\M P_{r, 0}^{-1}, \M P_{r, 0}>0$. 
\end{problem}
% By solving \Cref{prob:filter_batch}, we wish to obtain the minimizer $\{\hat{\M x}_0, \hat{\M x}_1, \cdots, \hat{\M x}_N \}$ th


% \begin{definition}[SOS belief]
% \label{def:SOS-factor}
% Given the estimation $\hat{\M x}$ and generalized covariance matrix $\M P$, the $r$-th order SOS belief is defined as:
%     \begin{equation}
%         \| \M \phi_r(\M x) - \M \phi_r(\hat{\M x}) \|^2_{\M P^{-1}}, \ \M P > 0.
%     \end{equation}
% % where the weighting matrix is the inverse of the equivalent generalized covariance of $\M \phi_r(\M x)$. % \tsl{Maybe call it prior SOS? }
% \end{definition}
% We will show that the SOS belief can be naturally obtained from the dual of \eqref{prob:pop_sdp} if a unique optimal solution is available.  

\subsection{Best Polynomial Unbiased Estimator}
\label{sec:BPUEdetails}

{\color{red} this needs more explanation and intuition. Also: you are assuming rank-1 before even introducing the SDP. }
% In the remainder of this paper, we make the following assumption to focus on the case that the \eqref{prob:pop_sdp} returns rank-one solutions:
% \begin{assumption}[Rank-one SDP]
% \label{assump:rank1sdp}
%     We assume that the solutions to the moment relaxations solved in this work satisfy the strict first-order optimality condition in \Cref{def:kkt_sdp}. 
% \end{assumption}
% Specifically, \Cref{prob:filter_batch} is a batched \eqref{prob:pop}.
 % \LC{unfortunately if modeling constraints is one the the key things we are trying to do, we cannot consider an unconstrained setup:} For simplicity, we consider the $\M x_{k}$ is unconstrained. 

%%%%% OLD VERSION %%%%%
% Analogous to the BLUE in linear dynamical systems with Gaussian noise \cite{kalman1960new, grewal2014kalman}, we derive the Best Polynomial Unbiased Estimator \eqref{eq:BPUE} \footnote{Note that the ``polynomial'' estimator here is a slight misnomer. In a linear system, BLUE is in the form of linear feedback. In our case, BPUE requires polynomial optimization to obtain the optimal estimation.} to estimate the monomials $\M \phi_r(\vxx)$ for the extended polynomial system in \eqref{eq:ext-polyDynSys}.
% It can be shown that the moment condition \eqref{gmm_condition} can be rearranged as an affine function of the basis $\M \phi_r(\M x)$: 
%%%%% OLD VERSION %%%%%

In this section, we introduce an estimator, Best Polynomial Unbiased Estimator \eqref{eq:BPUE}, to solve \Cref{prob:filter_batch}, borrowing ideas from the Best Linear Unbiased Estimator (BLUE) for linear systems.
First,

% In this section, we introduce an estimator, Best Polynomial Unbiased Estimator \eqref{eq:BPUE}, to solve \Cref{prob:filter_batch}, borrowing ideas from the Best Linear Unbiased Estimator (BLUE) for linear systems. To mimic BLUE, we first convert the polynomial conditions in \Cref{prob:filter_batch} into an affine combination of the monomial basis. 
% Then, we define \eqref{eq:BPUE} using the affine moment conditions of \eqref{add}. 

In \Cref{prob:filter_batch}, as the moment condition \eqref{gmm_condition} in the cost only contains polynomials, it adopts an affine form given the monomial basis $\M{\phi}_r(\M x)$. Thus, we mimic the BLUE to define the Best Polynomial Unbiased Estimator \eqref{eq:BPUE}\footnote{Note that the ``polynomial'' estimator here is a slight misnomer. In a linear system, BLUE is in the form of linear feedback. In our case, BPUE requires polynomial optimization to obtain the optimal estimation.} with this affine structure to study a class of state estimation problem as in \Cref{prob:filter_batch}. We first reformulate the moment condition \eqref{gmm_condition} to the following affine form: % Thus, we can extend the BLUE in linear systems \cite{kalman1960new, grewal2014kalman} to polynomial systems with a similar affine structure:

\begin{equation}
\label{eq:gmm_obs}
\begin{aligned}
    \boldsymbol m(\M y, \M x) &:= \vb(\M y) - \M{A}(\M y)\M \phi_r(\M x) \\
    \boldsymbol m(\M y, \bar{\M x}) &= \vv , \operatorname{Cov}[\vv] = \M V,
\end{aligned}
\end{equation}
where $\M{A}(\M y) \in \mathbb{R}^{m\times (s(n, r) - 1)}$ and $\vb(\M y) \in \mathbb{R}^{m\times 1}$ only contain the measurement $\M y$ and $\vv$ has zero mean. 

Note here that we slightly overload the notation $\M v$ to represent the higher-order monomials. Specifically, in the context of \eqref{eq:ext-polyDynSys}, $\M v := \M \phi_r(\vv) - \mathbb{E}\left[\M \phi_r(\vv)\right]$. We refer our readers to Appendix \ref{appx:momcond_linear} for examples of how to obtain \eqref{eq:gmm_obs} from moment conditions of the extended polynomial system. Then, we define \eqref{eq:BPUE} as the following \eqref{prob:pop} with the affine structure: % \tsl{Prove the unbiased, one sentence.}
%  In the framework of the generalized method of moments, the $\M m(\M y, \M x) = \M v$ is also called a moment condition since it is zero-mean.
\begin{definition}[Best Polynomial Unbiased Estimator] Consider the moment condition \eqref{eq:gmm_obs}, we define the BPUE with weighting matrix $\M W$ as:
\label{def:BPUE}
    \begin{equation}
    \label{eq:BPUE}
        \hat{\M x} = \argmin_{{\M x}\in \mathcal{K}}\quad \|\M b(\M y) - \M A(\M y)\M \phi_r(\M x)\|^2_{\M W} \tag{BPUE}
    \end{equation}
% \LC{these are claims and belong to a proposition/theorem, not to a "problem"}
As $\M v$ has zero mean when $\M x$ takes the true state $\bar{\M x}$, this estimator is unbiased \cite{hansen1982large, hayashi2011econometrics}. The optimal weighting matrix is taken when $\M W = \M V^{-1}$ \cite{hayashi2011econometrics, hansen1996finite}. % \tsl{Shall we add this sentence here?}
\end{definition}
Since \eqref{eq:BPUE} is no longer linear as in BLUE, there is no guarantee that $\hat{\M x}$ is globally optimal using local optimization techniques. However, the moment relaxation of \eqref{prob:pop} enables us to search for the globally optimal solution if rank-one relaxation is achieved. % \textcolor{blue}{(Ashkan: make sure to explain that moment relaxation and moments of uncertainties are two different things. At the beginning of section V, you can say that we will first formulate the estimation problem in terms of higher order moments of uncertainties. This will results in an nonlinear optimization problem. We then use SOS/moment relaxation to look for the optimal solution of the optimization problem. )}\david{we will change 'moment' earlier as 'monomials'/'terms' so that we will not use the term 'moments' in two scenarios but only in moment relaxation.} 
\tsl{We fixed the terms about the moments.}

{\color{red} This is still unclear. I agree with Ashkan's comment below}For the case $r = 1$, BPUE reduces to BLUE which is a quadratic program (QP). \tsl{How about adding the previous sentence?} In this linear Gaussian case, BLUE is equivalent to searching for the positive-definite quadratic form \cite{humpherys2012fresh} as a belief representation:
\begin{definition}[Quadratic Belief]
\label{def:SOS-factor}
Given the estimation $\hat{\M x}$ and the covariance $\hat{\M P} > 0$, the quadratic belief in Gaussian process is defined as:
    \begin{equation*}
        \| \M x - \hat{\M x} \|^2_{\hat{\M P}^{-1}}.
    \end{equation*}
\end{definition}
For \eqref{eq:BPUE}, We hereby consider the counterpart in polynomial systems as the following SOS polynomial: 
% We here extend the quadratic form to the following SOS polynomial associated with the rank-one optimal solution of the BPUE called SOS belief:
\begin{definition}[SOS Belief]
\label{def:SOS-factor}
Given the estimation $\hat{\M x}$ and $\hat{\M P} > 0$, the SOS belief $\sigma(\hat{\M x}, \hat{\M P})$ is an SOS polynomial defined as:
    \begin{equation*}
        \sigma(\hat{\M x}, \hat{\M P}) = \| \M \phi_r(\M x) - \M \phi_r(\hat{\M x}) \|^2_{\hat{\M P}^{-1}}.
    \end{equation*}
\end{definition}
\textcolor{blue}{(Ashkan: First explain the positive-definite quadratic form in BLUE before proving Def 5)  }\tsl{Resolved.}
The SOS belief is a generalization of the quadratic belief. % In \Cref{sec:theory}, we will show that the SOS belief can be naturally obtained from the dual of \eqref{prob:pop_sdp} and the weighting matrix $\hat{\M P} > 0$ is an approximated covariance of the $\M \phi_r(\hat{\M x})$. 

%%%%%%%
% PS should be simple, the rest goes into the Method

% Problem env should just be for the problem y want to solve

% others should be theorem/proposition

% SOS belief not clear, add explanation why it matters. filtering props the belief from t to t + 1, so we should include where the priors coming from

% Kalman gain never used

% consider a batch of measurement -- > say how BPUE is connected to 7 and 8

% 7 and 8 should be in method

% Predictioon --> prediction

% Two main issues: connection to BPUE. Theory results - explain WHY (example: Kalman gain)

% Approximate covariance part - not super clear

% contextualizing BPUE: 

%     story 1
%     problem formulation -- dyn sys, estimate from initial to current
%         what if we do batch from 0 to T. then introduce BPUE (just buncha measurements and then do estimation) --> is prior meaningful? (LC thinks batch is easier)
%         does not scale -> high-order -> do moment KF with two separate steps
%     story 2
%     formulation
%     GMM --> Why GMM? WHat is the point of BPUE...
    
%     OR if not say batch --> say let's start with UPDATE only



%     GMM separate section under method and justify WHY

%     BPUE whY: can solve via SDP relaxation -> can extract the prior via SDP but need to know what prior means, connect P in prior to BPUE.
   
%     if 
%     update using BPUE
%     Prediction
%     Marginalization

% Theory:
%     Justify prior vs dual
%     covariance approx

==> tex_v1/Abstract.tex <==
\begin{abstract}
    % We introduce a novel Generalized Moment Kalman Filter (GMKF) for polynomial systems corrupted by \emph{arbitrary} noise only assuming its moments are known. We first integrate the information in the higher-order moments of the noise by generating the polynomial dynamical system. We then extend the classical Best Linear Unbiased Estimator to the Best Polynomial Unbiased Estimator (BPUE) as a polynomial optimization problem (POP).  We show that the globally optimal solution of the BPUE can be obtained via the moment relaxation of POP. Under the assumption of rank-one solution of the moment relaxation, we derive the global optimality condition and find that the dual sum-of-square polynomial is an equivalence of uncertainty in moment space. Based on the theoretical analysis, we formulate the GMKF as a Weighted Least Square problem and derive the recursive solutions. We show that GMKF performs well under high non-normal noises. The proposed filter is evaluated on various robotics applications and outperforms the SOTA methods.
    % \tsl{Accessible}

    We introduce a novel filter for polynomial systems 
    %(i.e., dynamical systems described by polynomial equations) 
    corrupted by \emph{arbitrary} process and measurement noise. Given the moments of the noise, we formulate the filtering problem as a polynomial optimization problem (POP). The POP is then relaxed to a semidefinite program (SDP) via moment relaxation. Assuming the moment relaxation produces a rank-one solution, we derive the global optimality conditions and show that the estimated state can be extracted from the primal solution of the moment relaxation, while an approximate covariance can be computed from the dual solution.
    \red{LC: the following sentence is confusing: so far we were already claiming that we provide a filter}
    We further derive the Generalized Moment Kalman Filter as a recursive solution for the SDPs. We demonstrate that the filter performs well under highly non-Gaussian noise by evaluating it on various robotics applications and largely outperforms common alternatives.
    \red{LC: should we mention limitations? the abstract seems to overclaim}


\end{abstract}

==> tex_v1/BPUE-theory.tex <==
\section{Theoretical analysis of BPUE}
In this section, we derive the asymptotic property of the BPUE. We first show the equivalence between the rank-one optimal solution and a special class of sum-of-square polynomial certificate. Then we derive the generalized Kalman gain in SDP using the derived polynomial certificate. Finally, we provide the covariance of the estimated states. 

\subsection{Equivalence of SDP and SOS}
% We first introduce the theorem that moment relaxation \ref{prob:pop_sdp} is equivalent to having the prior factor when the strict KKT optimality condition is satisfied for the rank 1 optimal solution. 

% The main proof is inspired by \cite{cosse2021stable}, but we consider a more general case and do not introduce unnecessary variables in the primal problems. As such, we need $B$ and $B^{\perp}$ matrices. 

We introduce the following strict first-order optimality condition of \Cref{prob:pop_sdp} as a sufficient condition for unique rank-one solutions:
\begin{definition}[Optimality condition of rank-one \eqref{prob:pop_sdp}]
Consider the Lagrangian of \Cref{prob:pop_sdp} as 
%%%%%%%%%%%%%%%% inequality version %%%%%%%%%%%%%%%%
% \begin{equation}
% \begin{aligned}
%  L(X, Y, \Lambda) = &\langle C, X \rangle + \langle Y, X \rangle +  \sum_{i=0}^m \langle \Lambda_i, X \rangle \\
% &X \ge 0, Y \ge 0, \Lambda_i \ge 0
% \end{aligned}
% \end{equation}
%%%%%%%%%%%%%%%% equality version %%%%%%%%%%%%%%%%
\label{def:kkt_sdp}
\begin{equation}
\begin{aligned}
 L(\M X, \M Y, \M \lambda, \M \mu, \rho) = &\langle \M P, \M X \rangle - \langle \M Y, \M X \rangle +  \sum_{(i, \beta)} \M \lambda_{i, \beta} \langle \M G_{i, \beta}, \M X \rangle  \\
+ \sum_{(\gamma, \alpha)} \M \mu_{\gamma, \alpha} &\langle \M B^{\perp}_{\gamma, \alpha},  \M X\rangle  + \rho(1 - \langle \M e_1\M e_1^{\transpose}, \M X \rangle) % \\
% &X \ge 0, Y \ge 0.
\end{aligned}
\end{equation}
where $\M Y$, $\M \lambda$, $\M \mu$ and $\rho$ are the multipliers. By requiring that $\nabla_{\M X} L = 0$, feasibility of primal and dual problems, we have the following optimality condition:
\begin{enumerate}
    \item $\M Y = \M P + \sum_{(i, \beta)} \lambda_{i, \beta} \M G_{i, \beta} + \left( \sum_{(\gamma, \alpha)}\mu_{\gamma, \alpha} \M B^{\perp}_{\gamma, \alpha} - \rho \M e_1\M e_1^{\transpose} \right)$, % $L_{X} = 0\Rightarrow$
    \item $\M Y \ge 0, \M X \ge 0$, $\langle \M X, \M Y\rangle = 0$
    \item $\langle \M G_{i, \beta}, \M X \rangle = 0, \langle \M B^{\perp}_{\gamma, \alpha}, \M X \rangle = 0$, $\langle \M e_1\M e_1^{\transpose}, \M X \rangle = 1$,
\end{enumerate}
For a unique rank-one solution, it is sufficient to require the additional rank condition \cite{cosse2021stable}:
\begin{enumerate}[4)]
    \item $ Rank(\M X) = 1, Rank(\M Y) = s(\kappa, n) - 1$.
\end{enumerate}
\end{definition}

In the remainder of this paper, we make the following assumption to focus on the case that the \Cref{prob:pop_sdp} returns rank-one solutions:
\begin{assumption}[Rank-one SDP]
\label{assump:rank1sdp}
    We assume that the solutions to the moment relaxations solved in this work satisfy the strict first-order optimality condition in \Cref{def:kkt_sdp}. 
\end{assumption}

% Lemma \ref{lemma:exist_sos_xi} suggests that the two positive definite matrix constructs equivalent polynomials if their difference are linear combination of $\left\{ B^{\perp} \right\}$.
Inspired by \cite{cosse2021stable}, we derive the following Theorem that the optimality condition in \Cref{def:kkt_sdp} is equivalent to the existence of the prior factor:
\begin{theorem}[Equivalence of SDP and SOS]
\label{theorem:SDP=POP}
Suppose the unique optimal solution of \eqref{prob:pop} is $\bar{\M x}$, and the \eqref{prob:pop_sdp} corresponding to \eqref{prob:pop} has rank-one optimal solution $\M v_r(\bar{\M x})\M v_r(\bar{\M x})^{\transpose}$. Then there exists a dual certificate SOS
\begin{equation}
\begin{aligned}
    \sigma_0(\M x) &= \| \M \phi_r(\M x) - \M \phi_r(\bar{\M x}) \|_{\M W}^2  \\
    &= p(\M x) + \sum_{k=1}^m h_i(\M x)g_i(\M x) - \rho, \M W > 0
\end{aligned}
\end{equation}
% \mbox{$$}, $P>0$,
with $h_i(\M x)$ are polynomial multipliers, i.f.f the strict first order optimality condition \Cref{def:kkt_sdp} is satisfied. 
\end{theorem}
The detailed proof of \Cref{theorem:SDP=POP} is summarized in the Appendix. The proof is also a generalization of the result about the matrix completion problem in \cite{cosse2021stable}. 
Compared to \cite{cosse2021stable}, we use the $\{\M B^{\perp}\}$ to avoid additional multiplier to represent the monomials. 

\subsection{Generalized Kalman Gain}
% We consider $\M \phi_r(x)$ as independent variables to connect the KKT condition of SDP and the moment terms $m$. We consider the monomial as $m$, while they lie on the rank-one moment matrix. Thus we define $m_{e} = \left[1, \M \phi_r(m)\right]$ and the following quadratic constraints in appear in Problem \ref{prob:pop_sdp}:
% \begin{equation}
% \begin{aligned}
% m_em_e^{\intercal} = \begin{bmatrix}
%     1 & m^{\intercal} \\
%     m & mm^{\intercal} \\
% \end{bmatrix} \\
% \langle B_i^{\perp}, m_em_e^{\intercal}\rangle = 0. % , \langle e_1e^\intercal_1, m_em_e^{\intercal}\rangle = 1
% \end{aligned}
% \end{equation}
% Thus, we have the BPUE as the QCQP
% \begin{equation}
% \begin{aligned}
%     % \min_m\quad & \|\frac{1}{N}\sum_{k=1}^N A(y_k)m + b(y_k)\|^2_W \\
%     % \mathrm{s.t.}    &\langle B_i^{\perp}, m_em_e^{\intercal}\rangle = 0  we denote $\frac{1}{N}\sum_{k=1}^NA(y_k)$ and $\frac{1}{N}\sum_{k=1}^Nb(y_k)$ as $\hat{\M A}$ and $\hat{b}$, 
%     \min_m\quad & \| b(y) - A(y)m\|^2_W \\
%     \mathrm{s.t.}    &\langle B_i^{\perp}, m_em_e^{\intercal}\rangle = 0
%             % &\langle e_1e^\intercal_1, m_em_e^{\intercal}\rangle = 1
% \end{aligned}
% \end{equation}
For simplification, we omit the dependency of $\M A(\M y)$ and $\M b(\M y)$ on $\M y$ in \Cref{def:BPUE-QCQP}. Under the \Cref{assump:rank1sdp}, we can derive the local KKT condition of the \Cref{def:BPUE-QCQP}:
\begin{equation}
\label{eq:BPUE_local_kkt}
\begin{aligned}
    \min_{\M x} \max_{\M \mu}\quad L(\M m, \M \mu) = &\|\M b - \M A\M m\|^2_{\M W}  + \sum_i\mu_i\langle \M B_i^{\perp}, \M m_e\M m_e^{\intercal}\rangle  % // + \rho\left(\langle e_1e^\intercal_1, m_em_e^{\intercal}\rangle - 1\right)  \\
\end{aligned}
\end{equation}
For our analysis of the QCQP, we partition the $\M B^{\perp}$ to the first row $\M B^{\perp}_l$ and the remaining sub-principle matrix $\M B^{\perp}_Q$:
\begin{equation}
    \M B^{\perp} =: \begin{bmatrix}
        0 & \M B^{\perp \intercal}_{l} \\
        \M B^{\perp}_{l}& \M B^{\perp}_{Q} 
    \end{bmatrix}.
\end{equation}
Using the identical multiplier obtained in the \Cref{prob:pop_sdp}, we have the SOS as:
\begin{equation}
\begin{aligned}
    L(\M m, \M \mu) &= \M m_e^{\intercal}\hat{\M Y}\M m_e  + \hat{\rho} \\ % - \hat{\rho}
    % &= m^{\intercal}\hat{P}_em_e  + \hat{\rho} \\
    % % &= \langle P, mm^{\intercal} \rangle \\
    % &= \|m - \hat{\M m} \|^2_{\hat{P}}  + \hat{\rho}
\end{aligned}
\end{equation}
with the dual solution $\hat{Y}$:
\begin{equation}
\hat{\M Y} = \begin{bmatrix} \M b^{\transpose}\M W\M b - \hat{\rho} & (-{\M A}^{\intercal}\M W{\M b} + \sum_i{\mu}_i \M B^{\perp}_{l, i})^{\intercal} \\
        -{\M A}^{\intercal}\M W{\M b} + \sum_i{\mu}_i \M B^{\perp}_{l, i} & {\M A}^{\intercal}\M W{\M A} + \sum_i {\mu}_i\M B_{\M Q,i}^{\perp}
    \end{bmatrix}
    % \hat{Y} = \begin{bmatrix} (-{A}^{\intercal}W{b} + \sum_i{\mu}_i B^{\perp}_{l, i})^{\intercal}({A}^{\intercal}W{A} + \sum_i {\mu}_iB_{Q,i}^{\perp})^{-1}(-{A}^{\intercal}W{b} + \sum_i{\mu}_i B^{\perp}_{l, i}) & (-{A}^{\intercal}W{b} + \sum_i{\mu}_i B^{\perp}_{l, i})^{\intercal} \\
    %     -{A}^{\intercal}W{b} + \sum_i{\mu}_i B^{\perp}_{l, i} & {A}^{\intercal}W{A} + \sum_i {\mu}_iB_{Q,i}^{\perp}
    % \end{bmatrix}
\end{equation}
% \end{strip}
Then we have the local first-order optimality condition $\nabla_{\M m}L(\M m, \M \mu) = 0$ that is also globally certified:
\begin{equation}
    ({\M A}^{\intercal}\M W{\M A} + \sum_i {\mu}_i\M B_{Q,i}^{\perp})\M m - {\M A}^{\intercal}\M W{\M b} + \sum_i{\mu}_i \M B^{\perp}_{l, i} = 0
\end{equation}
Then we have the estimation as:
\begin{equation}
\begin{aligned}
    \hat{\M m} &= ({\M A}^{\intercal}\M W{\M A} + \sum_i {\mu}_i\M B_{Q,i}^{\perp})^{-1}({\M A}^{\intercal}\M W{\M b} - \sum_i{\mu}_i \M B^{\perp}_{l, i}) \\
            &= ({\M A}^{\intercal}\M W{\M A} + \sum_i {\mu}_i\M B_{Q,i}^{\perp})^{-1}\\
            &({\M A}^{\intercal}\M W(\M A\bar{\M m} + \M v) - \sum_i{\mu}_i \M B^{\perp}_{l, i})
\end{aligned}
\end{equation}
Then we can define the generalized BLUE with multipliers induced from the moment relaxation:
\begin{definition}[Gain of BPUE]
    $$\M K = (\M A^{\transpose}\M W\M A + \sum_i \mu_i \M B^{\perp}_{Q, i})^{-1}\M A^{\transpose}\M W$$
\end{definition}
Consider the Lagrangian of the SDP in the update steps with noiseless prior factor:
\begin{equation}
\label{eq:KF_local_kkt}
\begin{aligned}
    L(\M m, \M \mu) = & \|\M m - \hat{\M m}\|^2_{\M P} + \|\M b - \M A\M m\|^2_\M W \\
    &+ \sum_i\mu_i\langle \M B_i^{\perp}, \M m_e\M m_e^{\intercal}\rangle  % // + \rho\left(\langle e_1e^\intercal_1, m_em_e^{\intercal}\rangle - 1\right)  \\
\end{aligned}
\end{equation}
we can derive the generalized Kalman gain:
\begin{definition}[Generalized Kalman gain]
    $$\M K = (\M A^{\transpose}\M W\M A + \M P + \sum_i \mu_i \M B^{\perp}_{Q, i})^{-1}\M A^{\transpose}\M W$$
\end{definition}
\LC{also this is very unclear: we derive the gain K but that's not actually used by that algorithm?}
For the unconstrained linear optimal estimator, the multipliers vanish and degenerate to the BLUE and linear KF.  
% We find that for unconstrained cases, the result reduces to BLUE with the classical Kalman gain. \tsl{This is not Kalman gain... Kalman gain has a P matrix inside the ()}
% If we consider the cost function as in the update steps, we have the estimation as:
% \begin{equation}
% \begin{aligned}
%     \hat{\M m} &= ({A}^{\intercal}W{A} + P + \sum_i {\mu}_iB_{Q,i}^{\perp})^{-1}({A}^{\intercal}W{b} + Pm^{-} - \sum_i{\mu}_i B^{\perp}_{l, i}) \\
%             &=\bar{\M m} + ({A}^{\intercal}W{A} + P + \sum_i {\mu}_iB_{Q,i}^{\perp})^{-1}({A}^{\intercal}W(A\bar{\M m} + v) + Pm^{-} - \sum_i{\mu}_i B^{\perp}_{l, i}) \\
% \end{aligned}
% \end{equation}

\subsection{Approximated covariance of BPUE}
We extend the result of BLUE to polynomial systems and leverage the equivalence relationship in \Cref{lemma:exist_sos_xi} to show that the dual SOS is an approximated covariance of the estimation. Due to the nonconvexity of \Cref{def:BPUE-QCQP}, we fix the multipliers in the KKT condition \eqref{eq:BPUE_local_kkt} at an operating point. 

Consider the limiting noiseless case that:
\begin{equation}
    % \begin{aligned}
        \bar{\M A} := \mathbb{E}[\M A(\M y)], \bar{\M b} := \mathbb{E}[\M b(\M y)], \bar{\M A}\bar{\M m} = \bar{\M b}.
    % \end{aligned}
\end{equation}
We make the following assumption to enforce a sufficient condition for rank-one solution at the operating point:
\begin{assumption}[Observability]
\label{assump:observability}
    We assume that in the noiseless case, i.e. $\M A = \bar{\M A}$, $\bar{\M A}$ has full column rank to ensure unique recovery of the monomial $\M \phi_r(\bar{\M x})$. 
\end{assumption}
\begin{remark}
    Note that the observability analysis on the semialgebraic set is beyond the scope of this work, we assume this sufficient condition to guarantee the rank-one solution in this particular operating point. 
    \LC{unclear why the condition guarantees rank 1 for the SDP relaxation}
\end{remark}
For fixed $\mu = \bar{\mu}$ corresponding to this operating point, we have the perturbed solution given noise $v$ as: 
\begin{equation}
\hat{\M m} - \bar{\M m} = (\bar{\M A}^{\intercal}\M W\bar{\M A} + \sum_i \bar{\mu}_i\M B_{Q,i}^{\perp})^{-1}\bar{\M A}^{\intercal}\M W\M v
% \begin{aligned}
%     \hat{\M m} &= (\bar{A}^{\intercal}W\bar{A} + \sum_i \bar{\mu}_iB_{Q,i}^{\perp})^{-1}(\bar{A}^{\intercal}W{b} - \sum_i\bar{\mu}_i B^{\perp}_{l, i}) \\
%             &= (\bar{A}^{\intercal}W\bar{A} + \sum_i \bar{\mu}_iB_{Q,i}^{\perp})^{-1}(\bar{A}^{\intercal}W(\bar{A}\bar{\M m} + v) - \sum_i\bar{\mu}_i B^{\perp}_{l, i}) \\
%             &= \bar{\M m} + (\bar{A}^{\intercal}W\bar{A} + \sum_i \bar{\mu}_iB_{Q,i}^{\perp})^{-1}\bar{A}^{\intercal}Wv
% \end{aligned}
\end{equation}
Thus, we have the approximated covariance of the estimation:
\begin{equation}
    \operatorname{Cov}[\hat{\M m} - \bar{\M m}] =  \bar{\M P}^{-1}\bar{\M A}^{\intercal}\M W\M V\M W\bar{\M A}\bar{\M P}^{-1},
\end{equation}
with the $P$ evaluated at the limiting operating point:
\begin{equation}
    \bar{\M P} = (\bar{\M A}^{\intercal}\M W\bar{\M A} + \sum_i \bar{\mu}_i\M B_{Q,i}^{\perp}).
\end{equation}
% \david{Add theorem to include below two proofs}
Under \Cref{assump:observability}, a feasible dual multiplier is $\bar{\mu} = 0$. Thus, we can recover the covariance of BLUE at $\mu = 0$ as:
\begin{equation}
    \operatorname{Cov}[\hat{\M m} - \bar{\M m}] =  (\bar{\M A}^{\intercal}\M W\bar{\M A})^{-1}\bar{\M A}^{\intercal}\M W\M V\M W\bar{\M A}(\bar{\M A}^{\intercal}\M W\bar{\M A})^{-1}
\end{equation}
For the optimal weighting matrix $W = V^{-1}$, we have the covariance as:
\begin{equation}
    \operatorname{Cov}[\hat{\M m} - \bar{\M m}] =  (\bar{\M A}^{\intercal}\M V^{-1}\bar{\M A})^{-1} = \bar{\M P}
\end{equation}
When solving the moment relaxation, the dual certificate $P$ may not be identical to $A^{\transpose}V^{-1}A$ according to \Cref{lemma:exist_sos_xi}. However, \Cref{lemma:exist_sos_xi} also suggests that the dual certificate and the original cost function are equivalent as they correspond to identical polynomials. We then have the following theorem that provide theoretical support to our marginalization procedure in \Cref{def:gmkf_marginal} :
\begin{theorem}[Equivalent covariance in moment space]
\label{theorem:cov_mkf}
By \Cref{lemma:exist_sos_xi}, we can show that: $$\|\M \phi_r(\M x) - \M \phi_r(\bar{\M x})\|^2_{\M A^{\transpose}\M V^{-1}\M A} = \|\M \phi_r(\M x) - \M \phi_r(\bar{\M x})\|^2_{\M P^{-1}}$$
% \end{theorem}
% \begin{theorem}[Constrained equivalent covariance]
For the constrained case that $x_k \in \mathbb{K}$, we have the modified SOS certificate considering additional polynomial multipliers:
\begin{equation}
    \begin{aligned}
        \|\M \phi_r(\M x) - \M \phi_r(\bar{\M x})\|^2_{\M P^{-1}} &= \|\M \phi_r(\M x) - \M \phi_r(\bar{\M x})\|^2_{\M A^{\transpose}\M V^{-1}\M A} \\
        &\quad + \sum_i h_i(\M x)g_i(\M x)
    \end{aligned}
\end{equation}
For feasible point $\M x_k \in \mathbb{K}$, we must have $g_i(\M x_k) = 0$. Thus we have the equivalent generalized Gaussian on the support $\mathbb{K}$. 
% Thus, extracting the block in the propagation step is equivalent to obtaining the ``marginalized'' distribution in the moment space. % \tsl{How about the constrained case? We need to restrict the system on the support $\mathbb{K}$. }
\end{theorem}
Thus, extracting the block in the propagation step is equivalent to obtaining the ``marginalized'' distribution in the moment space. % \tsl{How about the constrained case? We need to restrict the system on the support $\mathbb{K}$

% However, it is worth noticing that the SOS obtained by the SDP and the cost function correspond to identical polynomials, which justifies that the dual solution of the SDP is a reasonable approximation of the covariance. 

==> tex_v1/Experiments.tex <==
\section{Numerical Experiments}
In order to demonstrate the efficacy of GMKF in real-world robotics applications, we design a variety of numerical experiments to evaluate its performance and compare our method with several baselines. We also respectively assess the performance of both the update and the propagation steps. 
\subsection{Comparison of BPUE and BLUE}
We first compare the result of BPUE with BLUE for linear systems. Though BLUE is optimal among all the linear feedback that provides minimal variance estimation, we show that BPUE which incorporates higher-order moments of the noise outperforms BLUE. 

We consider the linear observation $x, y \in \mathbb{R}^2$ function:
\begin{equation}
\begin{aligned}
    y_1 - x_1 &= v_1 \\
    y_2 - x_2 &= v_2
\end{aligned}
\end{equation}
and the noise $\M v \in \mathbb{R}^2$ with known moments. We consider the linear system corrupted by highly non-Gaussian noise. We consider a mixed Gaussian distribution with four peaks ...

We design a binary noise function and a trigonometric noise function, both of which are highly non-Gaussian. The binary noise is defined as follows:
\begin{equation}
    v_k = s\cdot\begin{bmatrix}
        \mathbb{I}(w_1>0)-0.5\\
        \mathbb{I}(w_2>0)-0.5
    \end{bmatrix} + \M \epsilon
\end{equation}
where $s$ is the scale factor, $w_1, w_2\sim 2\pi (Unif(0, 1)-0.5)$ and $\M \epsilon\sim \mathcal{N}(0, I)$. The trigonometric noise is defined as:
\begin{equation}
    v_k = s\cdot\begin{bmatrix}
    \cos(w\pi)\\
    \sin(w)
    \end{bmatrix}+ \M \epsilon
\end{equation}
where $w\sim 2\pi (Unif(0, 1)-0.5)$ and $\M \epsilon\sim \mathcal{N}(0, \M I)$.

% \subsection{BPUE vs. RLS}tf5
% \tsl{Do RLS 50 times, each 100 steps, and plot the log scale error. Both BLUE and BPUE. RLS is equivalent to batch using our method. }
% To separately evaluate the update step's performance, we compare the error of Recursive Least Squares (RLS) and BPUE under non-Gaussian noise. Specifically, we design two highly non-Gaussian noises: Binary and Trigonometric Noise, as shown in Fig. \ref{fig:binnoise} and \ref{fig:trignoise}. 

We plot the average error of 100 update steps under different noise scales ranging from 0.1 to 10. As illustrated in \Cref{fig:update-image1} and \Cref{fig:update-image2}, results suggest that under increasingly larger non-Gaussian noises, the BPUE estimates remain relatively consistent with a lower error increase rate than that of BLUE. 
\input{figs/update-only} \tsl{Need to point out the order of moments used in this formulation. }

% \subsection{Prediction Step}
\subsection{Covariance Propagation in Moment Space}
\harry{TODO: Banana shape gaussian, Cite the RSS paper.}
\harry{TODO: Prediction only: w/e is relevant, noise magnitude, number of est? Larger noise --> worse. Still makes sense to make it over time. not sure if it's relevant (consistency over time).}
Next, we separately assess the performance of the prediction step of GMKF.
% \subsection{Moment KF v.s. KF/UKF}

\subsection{Localization in $\mathrm{SE}(2)$}
We consider the localization of $\mathrm{SE}(2)$ systems with known landmarks. First, we define the dynamics on $\mathrm{SE}(2)$:
\begin{equation}
    \M X_{K+1} = \M X_k\M U_k\M W_k, 
\end{equation}
with $\M X_k$ the pose, $\M U_k$ the pose change and $\M W_k$ the dynamics noise, all defined on $\mathrm{SE}(2)$. For each $\mathrm{SE}(2)$ pose, we parameterize it as polynomial:
\begin{equation}
    \M X_k = \begin{bmatrix}
        c_k & -s_k & x_k \\
        s_k &  c_k & y_k \\
        0 &  0 & 1 \\
    \end{bmatrix}, c_k^2 + s_k^2 = 1.
\end{equation}
We consider the range-bearing observation function
\begin{equation}
    \M y_k = \M R_k^{\transpose}(\M p_L - \M p_k) + \M v_k. 
\end{equation}
where $\M R_k$ is the current step's rotation matrix, $\M p_L$ is the Cartesian coordinates of the landmark, $\M p_k$ is the current Cartesian coordinates of the robot, and $\M v_k$ is the observation noise. 
As the dynamics is corrupted by multiplicative noise, we approximate the covariance and obtain the process noise model via:
\begin{equation}
\begin{aligned}
    &\M X_{k+1} - \M X_k\M U_k = \bar{\M X}_k\bar{\M U}_k(\M W_k - \M I) \\
    &\M f(\M x_{k+1}, \M x_k, \M u_k) = \bar{\M U}_k^{\transpose}\bar{\M X}^{\transpose}_k(\M X_{k+1} - \M X_k\M U_k) = (\M W_k - \M I)
\end{aligned}
\end{equation}
where the operating point $\bar{\M X}_k$ is chosen as the most updated state $\hat{\M X}^{+}_k$. \tsl{Need to justify why this makes sense...}

A similar approximation is applied to the observation function and we obtain the observation noise model:
\begin{equation}
\begin{aligned}
    &\M R_k\M y_k - (\M p_L - \M p_k) =  \bar{\M R}_k\M v_k, \\ 
    &\M h(\M y_k, \M x_k) = \bar{\M R}^{\transpose}_k(\M R_k\M y_k - (\M p_L - \M p_k)) =  \M v_k. 
\end{aligned}
\end{equation}


\input{figs/mkf_vs_others}
We also compare the performance across different filters on highly non-linear systems under large non-Gaussian noises via the translation and rotation errors over time. We choose to compare with the Extended Kalman Filter (EKF), Unscented Kalman Filter (UKF), and the Invariant Extended Kalman Filter (InEKF) as the baselines. 

Moreover, we design a polynomial dynamical system that operates in $SE(2)$. Specifically, we make the system follow a circular trajectory in 2D with state representation of $(x, y, \cos(\theta), \sin(\theta))$. For each of the baselines, we fix the random seed and use the same noise functions to ensure fairness.

In \Cref{fig:mkf-image8}, we visualize the state estimates for each filter under both binary and trigonometric noises. We can see that due to the non-normality nature of the noises, all baselines failed to follow the circular trajectory consistently. Noticeably, the EKF baseline had the largest drift from the ground-truth trajectory.

We also report the average log-scale L2 error in meters for translation in \Cref{fig:trans-error} and the average log-scale angular difference in radians for rotation in \Cref{fig:rot-error} across 20 trials for each filter under the trigonometric noise. Again, GMKF had the lowest translation and rotation error across all filters and its performance stayed relatively consistent through the steps. While InEKF significantly outperformed other two baselines, it remained less accurate than GMKF.
\input{figs/trans-rot-error}



% \subsection{SE(2)}

% \clearpage

==> tex_v1/Formulation.tex <==
\section{Generalized Moment Kalman Filter}
\LC{this should be section IV, and BLUE should come after this}
% \harry{Need to move around and merge}
In this section, we derive the GMKF to utilize the information of noise in its higher-order moments. To achieve this goal, we first derive the extended polynomial dynamical system to enable the higher-order moments of noise to appear in the state space model. Then we develop the BPUE as a POP to extract the optimal state estimation. Finally, we formulate the filtering problem as the weighted least square. 

\subsection{Polynomial Dynamical System}
Consider the dynamical system of a deterministic parameter $\M x_{k}$ corrupted by i.i.d zero-mean random noise $\M w_k$ and $\M v_k$ with known moments:
% \david{move this to the front}
\begin{definition}[Polynomial dynamical system]
    \begin{equation}
    \label{eq:polyDynSys}
\left\{
	\begin{array}{l}
	\M f( \M x_{k+1}, \M x_{k}, \M u_k ) = \M w_k \\
	\ \ \ \M h( \M y_k, \M x_{k} ) = \M v_k
	\end{array},
		\M x_{k} \in \mathbb{K}, \M y_k \in \mathbb{R}^m.
\right.
\end{equation}
\end{definition}
where $\M f(\M x_{k+1}, \M x_{k}, \M u_k)$, the process model, and $\M h(\M y_k, \M x_{k})$, the observation model, are both polynomial functions. $\mathbb{K}$ is the support of $\M x_{k}$ defined by polynomial equality constraints. 

The classical Kalman filter assumes a linear dynamical system and uses moment information of the noise up to the second order, i.e. the mean and covariance. To utilize the higher-order moment of noise, we derive an extended polynomial dynamical system using the function $\M \phi_r(\cdot)$:
\begin{definition}[Extended polynomial dynamical system]
\begin{equation}
\begin{aligned}
    \label{eq:ext-polyDynSys}
    &\left\{
	\begin{array}{l}
	\M \phi_r\left(\M f( \M x_{k+1}, \M x_{k}, \M u_k )\right) - \mathbb{E}[\M \phi_r(\M w_k)] = \M \phi_r(\M w_k) - \mathbb{E}[\M \phi_r(\M w_k)] \\
	\M \phi_r\left(\M h( \M y_k, \M x_{k} )\right) - \mathbb{E}[\M \phi_r(\M v_k)] = \M \phi_r(\M v_k) - \mathbb{E}[\M \phi_r(\M v_k)] \\
 \quad \M x_{k} \in \mathbb{R}^n, \M x_{k} \in \mathbb{K}, \M y_k \in \mathbb{R}^m.
	\end{array}
\right. \\
\end{aligned}
\end{equation}
\end{definition}
It can be verified that the extended systems are corrupted by zero-mean noise. Now we compute the generalized covariance of the extended noise as:
\begin{equation}
\begin{aligned}
    \M R_r &:= \mathbb{E}\left[\left(\M \phi_r(\vv) - \mathbb{E}\left[\M \phi_r(\vv)\right]\right)\left(\M \phi_r(\vv) - \mathbb{E}\left[\M \phi_r(\vv)\right]\right)^{\transpose}  \right] \\
    \M Q_r &:= \mathbb{E}\left[\left(\M \phi_r(\vw) - \mathbb{E}\left[\M \phi_r(\vw)\right]\right)\left(\M \phi_r(\vw) - \mathbb{E}\left[\M \phi_r(\vw)\right]\right)^{\transpose}  \right]  
\end{aligned}
\label{RQdef}
\end{equation}

\subsection{Filtering in Moment Space}
% Thus, we consider the moment condition \eqref{eq:moment_condition} to design an efficient observer for this extended polynomial dynamical system. Consider the moment condition of the observation function: 
Given the extended polynomial dynamical system, we apply the BPUE to the observation and dynamics model:
\begin{equation}
\begin{aligned}
    \M m_{obs}(\M y_k, \M x_k) &:= \M \phi_r(\M h(\M y_k, \M x_k)) -  \mathbb{E}[\M \phi_r(\M v_k)] \\
    \M m_{dyn}(\M x_{k+1}, \M x_{k}, \M u_k) &= \M \phi_r(\M f(\M x_{k+1}, \M x_{k}, \M u_k)) - \mathbb{E}[\M \phi_r(\M w_k)]
\end{aligned}
\end{equation}
% It is obvious to see they have zero mean value when taking $\M x_{k}$ at the ground truth value $\bar{x}_k$. 

Consider $N$ inputs $\{\M u_0, \M u_1, \cdots, \M u_{N-1}\}$ and measurements $\{\M y_1, \M y_2, \cdots, \M y_N\}$, we formulate the BPUE for the extended state $\{\M x_0, \M x_1, \cdots, \M x_N\}$ with the following weighting matrix:
\begin{equation}
    W:= \{\M P^{-1}_{r, 0}, \M Q^{-1}_{r, 1}, \M R^{-1}_{r, 1}, \cdots, \M Q^{-1}_{r, N}, \M R^{-1}_{r, N}\}.
\end{equation}
\LC{everything should be correlated -- why this is a block diagonal matrix?}
Thus, we derive the batch optimization problem as the weighted least square problem:
\begin{problem}[Batch estimation in moment space] \LC{this makes a lot of sense, but it is confusing since we don't actually solve this problem}
    \begin{equation}
    \begin{aligned}
        \min_{ \{\M x_0, \M x_1, \dots, \M x_N \} }  \sum_{k=1}^{N} & \| \M m_{dyn}(\M x_{k-1}, \M x_{k}, \M u_k)\|^2_{\M Q^{-1}_{r, k}}
        + \| \M m_{obs}(\M y_k, \M x_{k})\|^2_{\M R^{-1}_{r, k}} \\
        + & \| \M \phi_r(\M x_0) - \M \phi_r(\hat{\M  x}_0)\|^2_{\M P^{-1}_{r, 0}} \\
        \mathrm{s.t.} & \quad \M x_{k} \in \mathbb{K}.
    \end{aligned}
\end{equation}
\end{problem}
The goal of this work is thus to derive a recursive solution to the batch problem as the GMKF. 
\LC{unfortunately if modeling constraints is one the key things we are trying to do, we cannot consider an unconstrained setup:} For simplicity, we consider the $\M x_{k}$ is unconstrained. 

% \section{GMKF Algorithm - from Theory to Practice}
% \section{Main Algorithm}
% TODO: Use some algorithm blocks. 
% 
\subsection{Recursive Implementation}
In this section, we introduce the main GMKF algorithm. We consider the recursive update of the prior factor shown in the \Cref{def:SOS-factor} given the measurement or the system input. 

\subsubsection{Initialization}

We initialize the prior factor given the generalized covariance $\hat{\M P}_0$ and initial estimation $\hat{\M x}_0$:
\begin{equation}
        \sigma_0(\M x) = \| \M \phi_r(\vxx_0) - \M \phi_r(\hat{\vxx}_0) \|^2_{\hat{\M  P}_0^{-1}}, \ \hat{\M  P}_0 > 0
\end{equation}

\subsubsection{Update}
We consider the update step given the most updated prior factor and observation in \eqref{eq:gmm_obs} and get an updated prior factor:
\begin{definition}[Update steps]
Given the prior factor at time $k$ and an observation $\M m_{obs}(\M y, \M x_{k})$ as in BPUE, we solve the \Cref{prob:pop_sdp} to get an updated prior factor:
\label{def:gmkf_update}
    \begin{equation}
    \begin{aligned}
        &\|\M \phi_r(\M x) - \M \phi_r(\hat{\M  x}^{+}_k)\|^{2}_{(\hat{\M  P}_k^{+})^{-1}} \\
        =& 
   \|\M \phi_r(\M x) - \M \phi_r(\hat{\M  x}_k^{-})\|^{2}_{(\hat{\M  P}_k^{-})^{-1}} + \|\M A(\M y_k)\M \phi_r(x) -\M b(\M y_k)\|^2_{\M R_k^{-1}}
    \end{aligned}
    \label{update}
    \end{equation}
\end{definition}

For the linear Gaussian case, the moment relaxation problem is equivalent to quadratic programming. For a comparison of the moment relaxation with KF, in terms of an update of covariance, please refer to the \Cref{appx:mkf_cov_update}.
% \tsl{This is not Kalman gain... Kalman gain has a P matrix inside the ()} \tsl{Operating point, A should be $\bar{A}$}
% We find that for unconstrained cases, the result reduces to BLUE with the classical Kalman gain. If we choose the operating point with noiseless measurement and prior, we have the equivalent propagation of covariance as:
% \begin{equation}
%     (\hat{P}^{+}_{k})^{-1} = (\hat{P}^{-}_{k})^{-1} + A^{\transpose}\M v_k^{-1}A  
% \end{equation}
% via the matrix inversion lemma, we can recover the classical result in Kalman filter:
% \begin{equation}
%     \hat{P}^{+}_k = \hat{P}^{-}_k - \hat{P}^{-}_kA^{\transpose}(\M v_k + A\hat{P}^{-}_kA^{\transpose})^{-1}A\hat{P}^{-}_k
% \end{equation}
% In the noisy case and assuming the rank one solution is available, we have the equivalent propagation of covariance considering the multiplier $\mu_i$ and the matrix $B^{\perp}$:
% \begin{equation}
%     (\hat{P}^{+}_{k})^{-1} = (\hat{P}^{-}_{k})^{-1} + A^{\transpose}\M v_k^{-1}A + \sum_i \mu_iB^{\perp}_{Q, i}
% \end{equation}
% \begin{equation}
%     \hat{P}^{+}_k = \hat{P}^{-}_k - \hat{P}^{-}_k\left((A^{\transpose}\M v_k^{-1}A + \sum_i \mu_iB^{\perp}_{Q, i})^{-1} + \hat{P}^{-}_k\right)^{-1}\hat{P}^{-}_k
%     \label{Cov_Update}
% \end{equation}
% We will show in the next section that the multipliers $\mu_i$ result in equivalent polynomials.
% % In either cases, the resulting polynomials are identical according to Lemma \ref{lemma:exist_sos_xi}. 

\subsubsection{Propagation}
In the propagation steps, we assume the knowledge of the prior factor and the system dynamics. Via solving the moment relaxation, we have the updated prior factor that contains the state at two consecutive steps:
\begin{definition}[Propagation steps]Given the prior factor at time $k$ and an input $\M u_k$ in the dynamics $\M m_{dyn}(\M x_{k+1}, \M x_{k}, \M u_k)$, we solve \Cref{prob:pop_sdp} to get an updated prior factor:
\label{def:gmkf_propagate}
    \begin{equation}
    \begin{aligned}
         &\|\M \phi_r([\M x_{k}, \M x_{k+1}]) - \M \phi_r([\hat{\M x}^{-}_k, \hat{\M x}^{-}_{k+1}])\|^{2}_{(\hat{\M P}_{k+1}^{-})^{-1}} \\
        =&\|\M \phi_r(\M x_{k}) - \M \phi_r(\hat{\M x}_k^{+})\|^{2}_{(\hat{\M P}_k^{+})^{-1}} + \|\M m_{dyn}(\M x_{k}, \M x_{k+1})\|^2_{\M Q_k^{-1}}
    \end{aligned}
    \label{propagation}
    \end{equation}
\end{definition}

Note that the propagation step provides the prior factor that involves the states in two consecutive time steps. To recursively update the state, we only keep the sub-principle matrix corresponding to $\M \phi_r(\M x_{k+1}) - \M \phi_r(\bar{x}_{k+1})$ as a mimic to the linear Gaussian case. To inherit convention in Bayes inference as in Kalman filter, we call this step marginalization though we do not explicitly define a distribution function:
\begin{definition}[Marginalization]
\label{def:gmkf_marginal}
    We partition $\M \phi_r([\M x_{k}, \M x_{k+1}])$ (up to permutation) to three parts
    \begin{equation}
        \M \phi_r([\M x_{k}, \M x_{k+1}]) := \begin{bmatrix}
            \M \phi_r(\M x_{k+1}) \\
            \M \phi_r(\M x_{k}) \\
            c(\M x_{k}, \M x_{k+1})
        \end{bmatrix}
    \end{equation}
    with the $c(\cdot, \cdot)$ denotes the cross term with the basis in two steps that appear in the same monomials. We also partition the information matrix as:
    \begin{equation}
    \begin{aligned}
        (\hat{\M P}^{-}_{k+1}) &=: \begin{bmatrix}
            \M P_{k+1, k+1} & \M P_{k+1, k} & \M P_{k+1, c} \\
            * & \M P_{k, k} & \M P_{k, c} \\
            * & * & \M P_{c, c} \\
        \end{bmatrix} \\
    \end{aligned}
    \end{equation}
    Then we only keep the sub-principle matrix corresponding to the state $\M x_{k+1}$:
    \begin{equation}
        (\hat{\M P}^{-}_{k+1})^{-1} \leftarrow \M P^{-1}_{k+1, k+1}
    \end{equation}
    To obtain the updated belief in the next step, we discard the cross terms and only keep the factor
    \begin{equation}
        \|\M \phi_r(\M x_{k+1}) - \M \phi_r(\hat{\M x}^{-}_{k+1})\|^2_{(\hat{\M P}^{-}_{k+1})^{-1}}
    \end{equation}
\end{definition}

\input{tex/General-Alg}
\begin{remark}[]
\LC{when r=1?}
In the unconstrained case linear, the problem is equivalent to computing the posterior covariance of Gaussian distribution. % \tsl{Maybe we need to only keep the algorithm block.}
\end{remark}

In the next section, we will show the connection of the proposed methods in polynomial systems with the linear Gaussian cases. We will show that the proposed method is a generalization of the classical Kalman filter.

==> tex_v1/General-Alg.tex <==
% \begin{algorithm}
% % \label{alg:general}

% \caption{Generalized Moment Kalman Filter Algorithm}\label{alg:mkf}

% \begin{algorithmic}
% \Require $r\gets$ the degree of moments, $\hat{P}_0 \gets$ generalized covariance, $\M f(x_{k+1}, x_k, \M u_k) = w_k \gets$ process noise model, $\M h(y_{k}, x_k) = v_k \gets$ observation noise model, $R_r, Q_r\gets$ generalized noise covariance \eqref{RQdef}. 
% \While{not $done$}

%     \State {$y_k \gets$ Observation}
%     \State {\texttt{// Update}}
%     \State {Solve Problem \ref{prob:gmkf_update}}
%     % \State {Solve for covariance update $\hat{P}_k^{+}$ via \eqref{Cov_Update}}
%     \State {\texttt{// Propagation}}
%     \State {Solve Problem \ref{prob:gmkf_propagate}}
%     \State {\texttt{// Marginalization}}
%     \State {Solve Problem \ref{prob:gmkf_marginal}}
%     \State $done \gets \texttt{FilteringDone}()$
% \EndWhile
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}
\label{alg:general}

\caption{Generalized Moment Kalman Filter}\label{alg:mkf}

\begin{algorithmic}
\Require $r\gets$ the degree of moments, $\hat{\M P}_0 \gets$ generalized state covariance, $\M f(\M x_{k+1}, \M x_k, \M u_k) = \M w_k \gets$ process noise model, $\M h(\M y_{k}, \M x_k) = \M v_k \gets$ observation noise model, $\M R_r, \M Q_r\gets$ generalized noise covariances \eqref{RQdef}. 
\While{true}
    \State {\texttt{// Prediction}}
    \State {Receive input $\M u_k$}
    \State {$\sigma\left([\hat{\M x}^{-}_k, \hat{\M x}^{-}_{k+1}]^{\transpose}, \hat{\M P}_{k+1}^{-}\right) \gets$ {\Cref{def:gmkf_predict}}}
    % \State {\texttt{// Marginalization}}
    \State {$\sigma\left(\hat{\M x}^{-}_{k+1}, \hat{\M P}^{-}_{k+1}\right)\gets$ {\Cref{def:gmkf_marginal}}}

    \State {\texttt{// Update}}
    \State {Receive observation $\M y_k$}
    \State {$\sigma\left(\hat{\M  x}^{+}_k, \hat{\M  P}_k^{+}\right)\gets${\Cref{def:gmkf_update}}}
\EndWhile
\end{algorithmic}
\end{algorithm}



% ********** TSL: If you need some reference **********

% \begin{algorithm}[t]
% \caption{\texttt{RRT-DCBF-MPC()}} %
% \small{
% \label{RRT-DCBF-MPC}
% \begin{algorithmic}[1]
% \Require Free space $\mathcal{X}_{f}$, start configuration $\bm{x}_{start}$;
% \State // Initialize node list, edge list, and tree
% \State $\mathcal{V}\leftarrow \{\bm{x}_{start}\}$; $\mathcal{E} \leftarrow \varnothing$
% \While{true} %
%     \State $\bm{x}_{rand} \leftarrow \texttt{Sample}(\mathcal{X}_f)$
%     \State $\bm{x}_{nearest} \leftarrow \texttt{Nearest}(\bm{x}_{rand},\mathcal{V})$
%     \State $\bm{x}_{new}$, isFeasible $\leftarrow \texttt{DCBF\_MPC}(\bm{x}_{nearest}, \bm{x}_{rand})$ % \leftarrow \text{DCBF_MPC}(\bm{X}_{nearest}, \bm{X}_{rand}, N);
%     \If{$\texttt{NoCollision}( \bm{x}_{nearest}, \bm{x}_{new}, \mathcal{X}_{f})$ \textbf{and} isFeasible}
%          \State  $\mathcal{E} \leftarrow \cup \{(\bm{x}_{nearest}, \bm{x}_{new})\}, \mathcal{V} \leftarrow \cup \{\bm{x}_{new}\}$
%          \If{\texttt{ReachGoal}($\bm{x}_{new}, \bm{x}_{goal}$)}
%             \State \textbf{break}
%          \EndIf
%     \EndIf
% \EndWhile
% \State \Return $\mathcal{T} = (\mathcal{V}, \mathcal{E})$ \\
% % \Function{Nearest}{G,$\bm{X}$}
% %     $\bm{X}_{nearest} \leftarrow \argmin  $
% % \EndFunction
% \Function{\texttt{DCBF\_MPC}}{$\bm{x}_{start}, \bm{x}_{goal}$}
%     \State $N \leftarrow \texttt{ComputeSteps}(\bm{x}_{nearest}, \bm{x}_{rand})$
%     \State $N \leftarrow \min(N, N_{max})$, $N \leftarrow \max(N, N_{min})$
%     \State $(\bm{x}_{1,2,...N}, \bm{u}_{0,1,2,...,N-1}$,isFeasible$)$ $\leftarrow \argmin$ Problem \ref{prob:Biped-DCBF-MPC}
%     \State $\bm{x}_{new} \leftarrow (\bm{x}_{1},\bm{u}_0)$
%     \State \Return $\bm{x}_{new}$, isFeasible
% \EndFunction
% \end{algorithmic}
% }
% \end{algorithm}


==> tex_v1/Math-Prelim.tex <==
\section{Preliminaries}
This section reviews key facts about polynomials and moment relaxations for the non-expert reader.
\LC{vectors and matrices must be in bold face}
% . Albeit being mathematically dense, these preliminaries serve as a quick introduction for non-expert readers.
\subsection{Polynomial and Moment Matrix}
Let $\mathbb{R}[x]$ be the ring of polynomial with real coefficients and $\vxx:=(x_1, x_2, \dots, x_n)$. Given an integer $r$, we define the set $ \mathbb{N}_r^n := \{\alpha \in \mathbb{N}^n | \sum_i \alpha_i \le r \}$ (i.e., $\alpha$ is a vector of integers that sums up to $r$). A monomial of degree up to $r$ is denoted as $x^{\alpha}:=x_1^{\alpha_1}x_2^{\alpha_2}\dots x_n^{\alpha_n}$, $ \alpha \in \mathbb{N}_r^n$. The canonical basis for polynomials  of degree up to $r$ is defined as:
\begin{equation}
\label{eq:basis}
    \vv_r(\M x):= (1, x_1, x_2,\dots,x_n, x_1^2,x_1x_2,\dots,x_n^2,x_1^r,x_2^r,\dots,x_n^r). 
\end{equation}
Let $s(r, n):=\begin{pmatrix}
    n+r \\ 
    n
\end{pmatrix}$ be the dimension of $\vv_r(\M x)$. We then define the polynomial function $\boldsymbol{\phi}_r(\M x): \mathbb{R}^{n} \rightarrow \mathbb{R}^{ s(r, n)- 1}$ using all the entries of the canonical basis except for $1$:
\begin{equation}
        {\M \phi}_r(\M x)= \begin{bmatrix}
        x_1, x_2,\dots,x_n, x_1^2,x_1x_2,\dots,x_n^2,x_1^r,x_2^r,\dots,x_n^r
        \end{bmatrix}. 
\end{equation}
Thus, the $r$-order rank-one moment matrix can be constructed:
\begin{equation}
    \M{M}_r(\M x) = \vv_r(\M x)\vv_r(\M x)^{\transpose}.
\end{equation}

\LC{do we really need all the preliminaries below? please check carefully and remove things that are not used}

% Given probability density function $\mu(\M x)$ on the support $\mathbb{K}$ \LC{K undefined}, we have the moment matrix of the distribution as:
% \begin{equation}
%     \M{M}_r(\M y) = \int_{x\in \mathbb{K}} \M{M}_r(\M x) \mu(\M x) d\M x.
% \end{equation}
% with 
% \begin{equation}
%     y_{\gamma} = \int_{x\in \mathbb{K}} x^{\gamma} \mu(x) d x
% \end{equation}

To construct a polynomial $p(\M x)$, we can extract the terms from $\M{M}_r(\M x)$ given a matrix $\M{P}$ and take the trace function as the inner product:
\begin{equation}
    p(\M x) = \operatorname{tr}(\M{P}\M{M}_r(\M x)) =: \langle \M{P}, \M{M}_r(\M x) \rangle
\end{equation}
We denote the degree, i.e., the highest order of monomial, of polynomial $g$ as $\operatorname{deg}g$. Then we have the \LC{$g_i$ undefined?} degree integers as $d_i := \left\lceil \operatorname{deg}(g_i) / 2 \right\rceil$ and $d_g = \max\{1, d_1,\dots,d_m\}$, where $\left\lceil a \right\rceil$ denotes the integer greater than or equal to $a$. Finally, we have the localizing matrix for polynomial $g(\M x)$:
\begin{equation}
    g(\M x)\M{M}_{r - \deg g}(\M x) = g(\M x) \vv_{r - \deg g}(\M x)\vv_{r - \deg g}^{\transpose}(\M x)
\end{equation}
\begin{equation}
    \begin{aligned}
    &\langle G_{\mu}, g(\M x)\M{M}_{r - \mathrm{deg}g}(\M x)(\alpha, \beta) \rangle = \sum_{\gamma} g_{\gamma}x^{\mu + \gamma}, \\
    &\alpha + \beta + \gamma \le s(2r, n),  \mu:=\alpha + \beta
    \end{aligned}
\end{equation}
\tsl{Check the definition of $G$.}
We now introduce two sets of matrix $\left\{\M{B}\right\}$ and $\left\{\M{B}^{\perp}\right\}$. We first introduce the auxiliary matrix $B_{\gamma}$ to form the moment matrix given the monomial $x^{\gamma}$:
\begin{equation}
    \M{B}_{\gamma} := \frac{1}{C_{\gamma}} \sum_{\gamma = \alpha + \beta} \ve_{\alpha} \ve^{\transpose}_{\beta},\ \  C_{\gamma}:= { \left| \left\{ (\alpha, \beta) | \gamma = \alpha + \beta \right\}  \right|  }
\end{equation}
where $\ve_\alpha \in \mathbb{R}^{s(r, n) \times 1}$ is the canonical basis corresponding to the $n$-tuples $\alpha \in \mathbb{N}_r^n$ and $C_{\gamma}$ is the normalizing factor. Thus, the moment matrix can be formulated by:
\begin{equation}
    \M{M}_r(\M x) = \sum_{\gamma} C_\gamma \M{B}_{\gamma} \M x^{\gamma}, \gamma \in \mathbb{N}^n_{2r}.
\end{equation}
% Conversely, we can extract the term of $\M{M}_r(y)$ via
% \begin{equation}
% x^{\gamma} = \langle B_\gamma, \M{M}_r(\M x) \rangle.
% \end{equation}
% We then define the orthogonal complement of $\left\{B\right\}$ considering the inner product as the trace function:
We define the symmetric matrix:
\begin{equation}
    \M{E}_{\alpha, \beta} = \ve_{\alpha}\ve_{\beta}^{\transpose} + \ve_{\beta}\ve_{\alpha}^{\transpose},
\end{equation}
and the orthogonal complement of $\left\{\M{B}\right\}$ to enforce the moment matrix constraints given an semidefinite matrix $X \ge 0$: 
\begin{equation}
   % \left\{ B^{\perp}_{\alpha, \beta} | \langle B^{\perp}_{\alpha, \beta}, B_{\alpha} \rangle, \forall \gamma \in \mathbb{N}^n_{2r} , \alpha + \beta = \gamma \right\}.
   \begin{aligned}
       &\M{B}^{\perp}_{\gamma, \alpha} = \M{E}_{\bar{\alpha}, \bar{\beta}} - \M{E}_{{\alpha}, {\beta}}, \\ 
       % &B^{\perp}_{\gamma, \alpha} = e_{\bar{\alpha}}e_{\bar{\beta}}^{\transpose} + e_{\bar{\beta}}e_{\bar{\alpha}}^{\transpose}  - e_{\alpha}e_{\beta}^{\transpose} - e_{\beta}e_{\alpha}^{\transpose}, \\ 
       &\alpha + \beta = \gamma, \alpha > \bar{\alpha}, \alpha \ge \beta, % \bar{\alpha} + \bar{\beta} = \gamma, 
   \end{aligned}
\end{equation}
where $\bar{\alpha} < \alpha$ is the tuple with the smallest possible lexical orders among all the $\alpha$. We provide a few examples of these matrices in \Cref{apx:B_mat_example}.
To assist the proof of our main theory, we introduce the following lemmas:
\begin{lemma}
\label{lemma:B_orthogonal}
    The set $\left\{\M{B}^{\perp}\right\}$ and $\left\{\M{B}\right\}$ forms a basis for matrix $\mathbb{R}^{s(r, n) \times s(r, n)}$ and they are orthogonal complements consider the matrix norm as trace function.
\end{lemma}
\begin{lemma}[Equivalent polynomial]
    \label{lemma:exist_sos_xi}
    Let $\M{Y}_1$ and $\M{Y}_2$ be two matrices such that $\vv^{\transpose}_r(\M x) \M{Y}_1 \vv^{\transpose}_r(\M x)=\vv^{\transpose}_r(\M x) \M{Y}_2 \vv^{\transpose}_r(\M x)$ for all $x$, i.e., the polynomials corresponding to $\M{Y}_1$ and $\M{Y}_2$ are identical. Then there exists a matrix ${\xi}$ with $\left\langle{\M{\xi}}, {\M{B}}_{{\gamma}}\right\rangle=0$ for all ${\gamma}$ such that $\M{Y}_1=\M{Y}_2+{\M{\xi}}$, $\M{\xi}=\sum_{(\gamma, \alpha)} \mu_{\gamma, \alpha} \M{B}^{\perp}_{\gamma, \alpha}$. % and $\xi = \sum_{(\gamma, \alpha)}\mu_{\gamma, \alpha}B_{\gamma, \alpha}^{\perp}$.
\end{lemma}
Given that the matrix $\M{Y} \ge 0$, we can define the following Sum-of-Square polynomial:
\begin{definition}[SOS polynomial]
    A sum of square (SOS) polynomial is defined as $$\sigma_0(\M x) = \sum_i h^2_i(\M x) =  \vv^{\transpose}_r(\M x)\M{Y}\vv_r(\M x), \M{Y} \ge 0.$$
\end{definition}

The proof of \Cref{lemma:B_orthogonal} and \Cref{lemma:exist_sos_xi} are presented in \Cref{apx:proof:B_orthogonal} and \Cref{apx:proof:exist_sos_xi}, respectively. In the abstract conic optimization setting, the result is more obvious and related to the null space of affine constraints, while we here consider the specific cone as the moment matrix. 
% The proof of Lemma \ref{lemma:exist_sos_xi} is inspired by \cite{cosse2021stable} but based on Lemma \ref{lemma:B_orthogonal} to construct the moment matrix.
% \begin{equation}
%     \M{M}_{r - \mathrm{deg}g}(gy) = \mathcal{L}_y(g(\M x)v_{r-\mathrm{deg}g}(\M x)v_{r-\mathrm{deg}g}(\M x)^{\transpose}).
% \end{equation}
% \begin{equation}
%     % G_{\gamma} = \sum_{\beta, \alpha} p_{\alpha}
%     % (gy)_{\gamma} = \sum_{\beta, \alpha} p_{\alpha}
%     \begin{aligned}
%     &\langle A_{\mu}, \M{M}_{r - \mathrm{deg}g}(gy)(\alpha, \beta) \rangle = \sum_{\gamma} g_{\gamma}y_{\mu + \gamma}, \\
%     &\alpha + \beta + \gamma \le s(2r, n),  \mu:=\alpha + \beta
%     \end{aligned}
% \end{equation}

\subsection{Polynomial Optimization}
% We define the following equality-constrained polynomial optimization for our moment matching problem:
We introduce the following equality-constrained polynomial optimization and its moment relaxation as a brief introduction to moment relaxation.
\begin{problem}[Equality-constrained POP]
\begin{equation}
\label{prob:pop}
\begin{aligned}
    % p^*&:=\inf p(\M x) \\
    % \mathrm{s.t.} \quad &g_j(\M x) = 0, \quad \forall j \in \{1,\ldots,m\}. \\
    p^* &= \inf_x \quad p(\M x) \\
    \mathrm{s.t.} \quad & g_j(\M x) = 0, \forall j \in \{1,\ldots,m\}. \\
\end{aligned}\tag{POP}
\end{equation}
We denote the feasible set as $\mathbb{K}$ and assume that $p(\M x) = \langle \M{P}, \M{M}_r(\M x) \rangle$. % We assume that $\mathbb{K}$ is compact. % \tsl{Add equality constraints or not.}
\end{problem}
We relax the moment matrix $\M{M}_r(\M x)$ by a semidefinite matrix $\M{X} \ge 0$ and enforce the linear moment matrix constraints using $\{\M{B}^{\perp}\}$. Note that $\vg(\M x) = 0$ implies $\vg(\M x)\M{M}_{r - \deg g}(\M x) = 0$, thus can leverage the definition of localizing matrix and derive the following moment relaxation problem:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We note that $\M{M}_r(\M x)$ is positive definite with the linear moment matrix constraints, thus, we can convert the \eqref{prob:pop} as a rank-one matrix optimization problem:
% \begin{problem}[Rank-one matrix optimization]
% \begin{equation}
% \begin{aligned}
% \label{prob:pop_sdp}
%     \rho_{\kappa}^*&:= \min_{X} \langle P, X \rangle \\
%     \mathrm{s.t.} \quad & X \ge 0, X_{1,1} = 1, \operatorname{Rank}(\M x) = 1 \\
%                   \quad & \langle B^{\perp}_{\gamma, \alpha}, X\rangle = 0, \gamma \in \mathbb{N}_{2\kappa}^n \\ % \text{Moment matrix structure} 
%                   \quad &\langle G_{i, \beta}, X\rangle = 0, i = 1, 2, \cdots, m
% \end{aligned}% \tag{SDP}
% \end{equation}
% The constraints at the first line encode the condition that the $X$ is PSD and normalized. 
% The constraint at the second line enforces the moment structure using the auxiliary matrix $B^{\perp}$. 
% The third constraint enforces the equality constraints by $g_i = 0$ via the localizing matrix. 
% \end{problem}
% As the rank condition is nonconvex, we discard it and finally have the moment relaxation of~\eqref{prob:pop}:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{problem}[Semidefinite relaxation of~\eqref{prob:pop}]
\label{prob:pop_sdp}
\begin{equation}
\begin{aligned}
    \rho^*&:= \inf_{\M{X}} \langle \M{P}, \M{X} \rangle \\
    \mathrm{s.t.} \quad & \M{X} \ge 0, \M{X}_{1,1} = 1\\
                  \quad & \langle \M{B}^{\perp}_{\gamma, \alpha}, \M{X}\rangle = 0, \gamma \in \mathbb{N}_{2\kappa}^n \\ % \text{Moment matrix structure} 
                  \quad &\langle \M{G}_{i, \beta}, \M{X}\rangle = 0, i = 1, 2, \cdots, m
\end{aligned}\tag{SDP}
\end{equation}
The constraints at the first line encode the condition that the $\M{X}$ is PSD and normalized. 
The constraint at the second line enforces the moment structure using the auxiliary matrix $\M{B}^{\perp}$. 
The third constraint enforces the equality constraints by $g_i = 0$ via the localizing matrix. 
\end{problem}
% \tsl{I am thinking about replacing rank-one matrix optimization with SOS.}
% Finally, we have the dual of \Cref{prob:pop_sdp} as the SOS optimization.
Moreover, solving the moment relaxation is equivalent to searching the SOS polynomial in the dual problem of \Cref{prob:pop_sdp}:
\begin{problem}[SOS programming]
\begin{equation}
\begin{aligned}
\label{prob:pop_sdp*}
    \rho^*&:=\sup_{\rho, \sigma_0, \{h_i \}} \rho \\
    \mathrm{s.t.} \quad &p(\M x) - \rho = \sigma_0(\M x) + \sum_{i=1}^{m} h_i(\M x)g_i(\M x)\\
    & \operatorname{deg} \sigma_0(\M x) \le 2{\kappa}, \operatorname{deg} \sigma_i g_i(\M x) \le 2{\kappa}.
\end{aligned}\tag{SOS}
\end{equation}
for some polynomial $\{h_i\}_{i=0}^{m}$ and SOS $\sigma_0$.
\end{problem}
\LC{ this seems to be a huge overclaim if we don't particularize it to our setup: 
The main theorem of this paper is to establish the relationship between the primal moment relaxation and its dual SOS optimization.} We show that the unique rank-one solutions to the \Cref{prob:pop_sdp} correspond to a special class of SOS polynomials that enable us to extract the unique state estimation. For an more complete introduction to moment relaxations in the view of measure theory, please refer to \cite{lasserre2015introduction}. 

% \subsection{Generalized Methods of Moment (GMM)}
% % \tsl{I am referring to Wiki.}
% Define $x \in \mathbb{R}^n$, the unknown parameter we wish to estimate, and $y_k$ the measurement. We denote the true value of $x$ as $x_0$. The GMM requires the moment condition to be satisfied: 
% \begin{equation}
% \label{eq:moment_condition}
%     \bar{g}(x_0) := \mathbb{E}\left[ g(y_k, x_0) \right] = 0,
% \end{equation}
% where $m(y_k, x)$ is a vector-valued function that relates the measurements and parameters to be estimated. 

% By the assumption that $y_k$ is generated by a weakly stationary ergodic stochastic process, we have the estimation of $m(x_0)$ by:
% \begin{equation}
%     \hat{g}(x_0) = \frac{1}{N}\sum_{k=1}^N g(\M x). 
% \end{equation}
% Then, the GMM estimator can written as:
% \begin{equation}
%     \hat{x} = \argmin_x \sum_{k=1}^N \left(\frac{1}{N}g(y_k, x)^{\transpose}\right)W\left(\frac{1}{N}g(y_k, x)\right), 
% \end{equation}
% with $W > 0$ a positive definite matrix. 
% The GMM estimator is consistent in the sense that: $$N \rightarrow \infty \Rightarrow x \rightarrow x_0. $$
% We then define the generalized covariance matrix 
% \begin{equation}
%     \Omega := \mathbb{E}\left[g(y_k, x_0)g(y_k, x_0)^{\transpose}\right] .
% \end{equation}
% The GMM is most efficient when the weighting matrix 
% \begin{equation}
%     W \propto \Omega^{-1}. 
% \end{equation}

% Consider the point estimation problem for the measurement:
% \begin{equation}
%     y_k = h(\M x) + v_k, k = 1, 2, \dots, N.
% \end{equation}
% \tsl{Note the order.}

% The GMM methods suggest that:
% \begin{equation}
% \begin{aligned}
%     \hat{x} &= \argmin_x \sum_{k=1}^{N} \| m_k(\M x) \|^2_{W_k} \\
%     &= \argmin_x \langle M(\M x) - M(v), M(\M x) - M(v)  \rangle_{W}
% \end{aligned}
% \end{equation}
% with
% \begin{equation}
% \begin{aligned}
%     m_k(\M x)&:= v_r\left(y_k - h(\M x)\right) - \mathbb{E}\left[v_r(v_k)\right] \\ 
% \end{aligned}
% \end{equation}
% This formulation requires us to match each monomial in the moment matrix. 

% The optimal weighting matrix takes the form:

% $$
% W^{-1}_k:=\mathbb{E}\left[ m_k(\M x)m_k(\M x)^{\transpose} \right]
% $$

% \tsl{If we only match the mean of $m$, we need covariance of $v_r$ to match. }
